Challenges and Opportunities in the Co-design of Convolutions and RISC-V Vector Processors

The RISC-V "V" extension introduces vector processing to the RISC-V architecture. Unlike most SIMD extensions, it supports long vectors which can result in significant improvement of multiple applications. In this paper, we present our ongoing research to implement and optimize a vectorized Winograd algorithm used in convolutional layers on RISC-V Vector(RISC-VV) processors. Our study identifies effective techniques for optimizing the kernels of Winograd on RISC-VV using intrinsic instructions, and showcases how certain instructions offer better performance. Our co-design findings suggest that the Winograd algorithm benefits from vector lengths up to 2048 bits and cache sizes up to 64MB. We use our experience with Winograd to highlight potential enhancements for the standard that would simplify code generation and aid low-level programming. Finally, we share our experience from experimenting with forks of gem5 for RISC-VV and stress the importance of a mature software ecosystem, to facilitate design space exploration and architectural optimization.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Winograd-old.tex <==
We use YOLOv3, a convolutional-based neural network for object detection, based on the convolutional layers with 1$\times$1 and 3$\times$3 kernel sizes. We use the Winograd algorithm for the convolutional layers with 3$\times$3 kernel size with stride 1 and im2col+GEMM for the rest of the layers and we call it \emph{hybrid approach}. We then compare the performance achieved by the hybrid approach compared to the im2col+GEMM approach, where im2col+GEMM implementation is used for all the layers. To keep the time within bounds, we simulate only the first 20 layers, out of which 15 are the convolutional layers. \sonia{We note a $\sim$8\% improvement in performance when using the hybrid approach compared to the im2col+GEMM approach when running with 2048-bit vector length with 1MB of L2 cache size using gem5~\cite{plct-gem5}, which also means the Winograd algorithm runs faster compared to im2col+GEMM on RISC-VV. The reason for this very less improvement is that from the first 20 layers, 15 are the convolutional layers. Out of these 15 layers, 3 layers are with stride 2, 6 layers are with 1x1 kernel size and the very first layer has the number of channels as 3. Therefore, the remaining 5 layers contribute to improving the performance.We also compare the performance achieved on RISC-VV and ARM-SVE, we observed that Winograd on RISC-VV performs the same as on ARM-SVE.}
\deleted{We observe less number of instructions in the case of the hybrid approach and $\sim 2 \times$ CPI (cycles per instruction) compared to the im2col+GEMM approach on RISC-VV. To investigate the cause of this, we examine the statistics produced by gem5 simulations, analyze the intrinsics used for vectorizing the kernels and also analyze the produced assembly codes. }


%and also we analysed the intrinsics the 
%We note a performance drop of 1.4X after using the Winograd implementation for the layer with 3x3 kernel size and stride 1. To know the reason behind this, we analyze the statistics generated from the implementation where all the layers use only the im2col+gemm algorithm and from the implementation where the Winograd algorithm is being used for the layers with 3x3 kernel size and stride 1. 

 One of the main reasons behind this is the use of indexed load instructions in tuple multiplication to load the quadword (4$\times$ 32-bit data) from memory to the vector register, which is a cycle-intensive instruction in terms of cycles, thereby affecting overall performance. To the best of our knowledge, the support for loading the quadword data from memory to the vector register is not available in the "V"  extension of RISC-V. On the other hand, we have a specific intrinsic instruction \texttt{svld1rq} to load the quadword data from memory to vector registers in ARM-SVE. To investigate this, we conducted a brief experiment where we replicated the index vector load to pack the quadword in the vector register and compared its performance to using the intrinsic 
\texttt{svld1rq} available for loading the quadword in the entire vector register on ARM-SVE.  Our results revealed a 2$\times$ performance drop with the indexed vector load on the A64FX machine. therefore, integrating quadword reading functionality can help in enhancing the performance further. 

The second reason is the register spilling due to the use of the vector register to store intermediate vector operations. The NNPACK implementation of the Winograd algorithm employs 16 vector registers by processing an 8$\times$8 input tile. The algorithm performs transformations on the loaded vector registers and stores the outputs in temporary vector registers. These transformations are utilized repeatedly within the function on various input vector data. However, since it's not possible to pass the vectors as a reference to the function, the transformations must be incorporated inside the main function, making the programming error-prone and challenging for developers to optimize the use of the temporary vector registers, triggering the vector register spilling. Therefore, it becomes a hurdle in improving performance. On the other hand, this is not the limitation with ARM-SVE, which makes programming cleaner and no spilling in registers has been observed. Therefore, having pointers with vector data type will not only improve programmability but also will help in reducing the chances of register spilling, resulting performance boost. 

Further, to transpose four vectors in RISC-VV, store and gather-load operations are necessary since there are no specific custom instructions in the "V" extension available for this task. However, ARM-SVE provides specific instructions to create an array of vectors and store them in memory with transposed vector data, which still requires storing and loading operations to transpose the vector data. In our experiment, we compared the performance of replicating the store and gather-load instructions for transposing the four vectors to using the combination of specific intrinsic instructions \texttt{svcreate4} and \texttt{svst4} on ARM-SVE. Our results revealed a drop in performance when using the specific intrinsics on A64FX, and suggests that \texttt{svcreate4} and \texttt{svst4} are even more cycle-intensive. Thus, we conclude that having a custom extension for transposing with 4 vectors without the need for memory operation in the "V" extension of RISC-V can boost performance.


Further, we performed the co-design study to assess the impact on performance by tuning the hardware parameters of RISC-VV using the gem5 simulator. With this fork of the gem5 simulator for RISC-VV, we were able to perform the simulations only up to 4096-bit vector length. Also, we used SPIKE, an emulator for RISC-VV, for validating our implementation, also supports up to 4096-bit vector length. Therefore, we are presenting our results analysis up to 4096-bit vector lengths. As shown in the figure~\ref{fig:YOLOV3longercachewinograd}, we can see a speedup of $\sim$1.4$\times$ from 512-bit vector length to 4096-bit vector length. Along with indexed load and spilling, L2 cache miss rate is another factor that limits the scalability with longer vector lengths. Further, we can see a total speedup of $\sim$1.4$\times$ from 1MB of L2 cache to 64MB of L2 cache. Beyond 64MB of cache, no significant performance improvement is observed. This concludes that our Winograd implementation does not require bigger L2 caches and this also validates the conclusion that we observed while working with ARM-SVE.  
%We do not see a performance benefit from 64MB to 256 MB. 



% Shall we include this?
%In total, there are 3 convolutional layers with 3x3 kernel size with stride 2, which have an input or output channel of 32, which allows the utilization of 4096-bit vector length vector registers. For vectorizing the tuple multiplication, we increase the number of blocks in the GEMM kernel, using 64 blocks with 4 elements in each block. We, therefore, can utilize the maximum of 8192-bit vector length in the tuple multiplication kernel. 



%For the Winograd implementation, we use inter-tile parallelization across the input/output by taking 8x8 tiles from each channel. 





%we use the Gem5 simulator for analyzing the performance using our Winograd implementation with different hardware parameters tuning. Figure\ref{YOLOV3longercachearmsvewinograd} presents the performance analysis for Winograd implementation for RISC-VV. From 512-bit to 4096-bit, we get $\sim$ 1.7X improvement, while from 1MB to 256MB cache, we get $\sim$ 1.2X performance improvement. 

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/yolov3-20layers-Latest-WinogradConstantLat.pdf}
  \caption{
  Impact of vector lengths and L2 cache size with Winograd on RISC-VV@gem5 for YOLOv3.}
  \label{fig:YOLOV3longercachewinograd}
  \vspace{-1.3em}
\end{figure}



==> programmability-old.tex <==

%The "V" extension of RISC-V provides the vector processing capability where architecture can have a vector length of up to 16384-bit. The compiler provides  the capability to vectorize to auto-vectorize the kernels. 

As discussed in Section~\ref{background}, we have used an inter-tile parallelism approach across the input/output channels, to vectorize the Winograd algorithm for longer vector lengths. In this approach, we use 8$\times8$ tiles from 4 channels to utilize 512-bit vector registers. In this way, to utilize 8192-bit vector lengths, we need to use 64 channels. In the convolutional layers where the number of channels is more than 4, we enable inter-tile parallelism for RISC-VV. Further, to vectorize the tuple multiplication, which can employ up to 8192-bit-long vectors, we now increase the number of blocks to 64, with 4 elements in each block. Thus, we can vectorize and use the Winograd algorithm with long vectors with RISC-VV. The vector extension of the RISC-V ISA offers a diverse range of EPI built-ins that enable manual kernel vectorization. We use these EPI built-ins for the manual vectorization of all the kernels in the Winograd algorithm on RISC-VV. 
%These instructions provide clear guidance on utilizing built-ins to vectorize kernels. 

\sonia{During the process of manually vectorizing with intrinsic instructions, as well as in our evaluation (see Section~\ref{results}, we demonstrate the use of effective available RISC-VV intrinsic instructions for vectorizing the Winograd kernels.  We also identified shortcomings in the RISC-V "V" extension, which would otherwise boost programmability. }

\deleted{However, during the process of manually vectorizing with intrinsic instructions, as well as in our evaluation (see Section~\ref{results},  we identified the following shortcomings in the RISC-V "V" extension, which would otherwise boost both programming productivity and performance:}

\begin{enumerate}
    \item[(i)]  In the input transformation kernels of Winograd, approximately 30 lines of code used for transforming the input data and producing the transformed output need to be used at %around 
    6 places, with different input data sets.  These instructions produce the intermediate output before producing the final, transformed output. In this scenario, it would be more practical to incorporate these instructions into a function and invoke it whenever transformation is necessary. However, this function must update output registers with the transformed output, thus requiring that output registers be passed as a reference. While optimizing the input transformations using manual vectorization on RISC-VV, we are forced to incorporate these 30 lines of code in the main function only at 6 different places, making the function lengthy, error-prone, and less efficient. Similarly to input transformation, we observe the same in kernel transformation and output transformation. This diminishes the readability of the code, making it difficult to reuse/modify. This also requires using all the intermediate vector registers in one place, triggering vector register spilling. It is not always possible for programmers to optimize the use of the intermediate vector registers to avoid vector register spilling. 
    \deleted{On the other hand, ARM-SVE provides the functionality to pass the vector register as a reference, resulting in avoiding the chances of register spilling and more clean programming.} 
    %Therefore, it becomes a hurdle in improving the performance and also diminishes the readability of the code, and makes it difficult to reuse/modify. 
    As a result, we conclude that having pointers with vector data types in the "V" extension will improve the programmability and will also help reduce the chances of register spilling.
    
    %While working with ARM-SVE, we get this feature where we can pass the address of vector registers and update the values on their addresses based on the calculations. However, while working with RISC-VV, we note that this feature is not present, and because of this many instructions ended up lying in the same kernel making the kernel very big and error-prone and can cause register spilling due to intermediate buffers. This not only impact on the performance but also diminishes the readability of the code and makes it difficult to reuse/modify. 

\begin{algorithm}[]
\caption{Tuple multiplication code snippet from Winograd showcasing the indexed load work-around in RISC-VV}

\begin{algorithmic}[1]

\STATE $ind\gets 0$ 
\STATE  VL = get vector length
\STATE $elements = 4$
\STATE $rem = VL/elements$
\STATE $num\gets blocks*4$ //64 blocks
\STATE $iteration\gets num/64$ 
\FOR{$i\gets 0$, $i<rem$, $i+=1$}
\FOR{$j\gets 0$, $j<4$, $j+=1$}
\STATE $index[ind] = j$
\STATE $ind++$;
\ENDFOR
\ENDFOR

\FOR{$itr\gets 0$, $itr<num$ }
        \STATE $gvl = setvl(num-itr)$
        \STATE $index\_vec\gets index[0:gvl]$
        \FOR{$k\gets0$, $k<iteration$, $k+=1$}
        \FOR{$j\gets 0$, $j< inputchannels$, $j+=1$}
            \STATE $b0\_vec \gets B[itr+(j*VL)]$ //load filter matrix
            \FOR{$i\gets 0$, $i<64$, $i+=4$}
            \STATE $a0\_vec \gets indexed\_load(A[(i+(64*k))+(j*VL)],index\_vec, gvl])$
            \STATE $acc\_vec[i] \gets vfmacc(acc\_vec[i], a0\_vec, b0\_vec, gvl)$
        \ENDFOR
        \ENDFOR
        \STATE Store results in the resultant matrix in a contiguous way
    \ENDFOR
    \STATE itr+=gvl;
\ENDFOR
\end{algorithmic}
\label{algo:winogradRISCVV}
\end{algorithm}

\begin{algorithm}[]
\caption{Tuple multiplication code snippet from Winograd using the slideup instructions in RISC-VV}
\begin{algorithmic}[1]

\STATE $ind\gets 0$ 
\STATE  VL = get vector length
\STATE $iteration\gets num/64$ 
\FOR{$itr\gets 0$, $itr<num$ }
        \STATE $gvl = setvl(num-itr)$
        \STATE $index\_vec\gets index[0:gvl]$
        \FOR{$k\gets0$, $k<iteration$, $k+=1$}
        \FOR{$j\gets 0$, $j< inputchannels$, $j+=1$}
            \STATE $b0\_vec \gets B[itr+(j*VL)]$ //load filter matrix
            \FOR{$i\gets 0$, $i<64$, $i+=4$}
            \STATE $a0\_vec \gets load(A[(i+(64*k))+(j*VL)], gvl])$
            \FOR{$ind\gets0$, $4*ind<=gvl/2$, $ind+=1$}
                \STATE $a0\_vec \gets Slideup(a0\_vec, 4*ind, gvl)$
            \ENDFOR
            \STATE $acc\_vec[i] \gets vfmacc(acc\_vec[i], a0\_vec, b0\_vec, gvl)$
        \ENDFOR
        \ENDFOR
        \STATE Store results in the resultant matrix in a contiguous way
    \ENDFOR
    \STATE itr+=gvl;
\ENDFOR
\end{algorithmic}
\label{algo:winogradRISCVVSlideup}
\end{algorithm}

\begin{algorithm}[]
\caption{Tuple multiplication code snippet from Winograd for ARM-SVE}
\begin{algorithmic}[1]
\STATE  VL = get vector length
\STATE $num =blocks*4$ //16 blocks 
\FOR{$itr\gets 0$, $itr<num$, $itr+=svcntw()$}
        \STATE $pg = svwhilelt\_b32(VL)$
       \FOR{$j\gets 0$, $j< inputchannels$, $j+=1$}
        
            \STATE $b0\_vec \gets B[itr+(j*VL)]$ //load filter matrix
            \FOR{$i\gets 0$, $i<64$, $i+=4$}
τ            \STATE $a0\_vec \gets svld1rq(pg, A[i+(j*VL)])$
            \STATE $acc\_vec[i] \gets svmla\_m(pg, acc\_vec[i], a0\_vec, b0\_vec)$
        \ENDFOR
  
        \STATE Store results in the resultant matrix in a contiguous way
    \ENDFOR
\ENDFOR

\end{algorithmic}
\label{algo:winogradARMSVE}
\end{algorithm}


\begin{algorithm}[]
\caption{Transpose code snippet from Winograd for ARM-SVE}
\begin{algorithmic}[1]
\STATE $VL\gets svcntw()$ // get vector length
\STATE $V0, V1, V2, V3$ //Vector registers
\STATE svfloat32x4\_t $inp0123\gets svcreate4(V0, V1, V2, V3)$
\STATE  $qin0123[4*VL]\gets 0$
\STATE $svst4(pg, \&qin0123[0] , inp0123 )$
\STATE $trans\_vec1[0:VL]\gets load(pg, \&qin0123[0], index)$
\end{algorithmic}
\label{algo:transposeARMSVE}
\end{algorithm}

\begin{algorithm}[]
\caption{Transpose code snippet from Winograd for RISC-VV}
\begin{algorithmic}[1]
\STATE $VL$ = vector length
\STATE $gvl$ = granted vector length
\STATE $V0, V1, V2, V3$ //Vector registers
\STATE $vin0123[0]\gets V0$
\STATE $vin0123[VL]\gets V1$
\STATE $vin0123[2*VL]\gets V2$
\STATE $vin0123[3*VL]\gets V3$
\STATE $ind\gets 0$ 
\FOR{$j = 0$, $j < 4$, $j+=1$}
\STATE $index[ind] = ((j * VL))$
\STATE $ind++$
\ENDFOR
\STATE  load index in $index\_vec$
\STATE $trans\_vec[0:gvl]\gets indexed\_load(\&vin0123[0], index\_vec, gvl)$
\end{algorithmic}
\label{algo:transposeriscvv}
\end{algorithm}


    \item[(ii)] In the tuple multiplication kernel from the Winograd algorithm, the logic requires reading a block of 4$\times$ 32-bit elements (quadword) for the transformed input matrix, to perform the element-wise multiplication with the loaded transformed filter matrix. 
    \sonia{While vectorizing the tuple multiplication kernel with RISC-VV, we are trying to use the best suitable existing intrinsic instructions to fill the vector register from the quadword, as there is no specific intrinsic available to perform this task. At first, we used the indexed vector load to fill the vector register from quadcore, and from figure~\ref{fig:tuplemult}, we can see the example of using the indexed vector load to pack the quadword in a 512-bit vector register. The code snippet in the algorithm~\ref{algo:winogradRISCVV}, presents our implementation of tuple multiplication using indexed vector load on RISC-VV. In line 18, we employ an indexed vector load operation to retrieve a quadword from the $A$ matrix. To use the indexed vector load, we generate indices in lines 5 to 10 and load them into the index vector $index\_vec$. We then utilize the index vector as the second argument when loading data from the $A$ matrix to the $a0\_vec$ vector register. However, the scatter and gather instructions are very expensive, therefore, we used another available intrinsic instruction i.e. slide-up to pack the vector register with quadword data as shown in the figure~\ref{fig:slideup}. The code snippet in the algorithm~\ref{algo:winogradRISCVVSlideup}, presents our implementation of tuple multiplication using slideup intrinsic instructions on RISC-VV. In line 10, we use a vector load operation to retrieve data from the $A$ matrix in the $a0\_vec$ vector register. Then we use the slideup intrinsic instructions from line 12 to line 14 to fill the vector with quadword data. After comparing the test snippets implemented with both the algorithms for the tuple multiplications for 100 iterations, we note that tuple multiplication using slideup intrinsic instructions is $\sim$2.3$\times$ faster than tuple multiplication using indexed intrinsic instructions.  }
    
    \deleted{While vectorizing the tuple multiplication kernel with RISC-VV, we are forced to use the indexed vector load to fill the vector register from the quadword, as there is no specific intrinsic available to perform this task. From figure~\ref{fig:tuplemult}, we can see the example of using the indexed vector load to pack the quadword in a 512-bit vector register. The code snippet in the algorithm\ref{algo:winogradRISCVV}, present our implementation of tuple multiplication on RISC-VV. In line 18, we employ an indexed vector load operation to retrieve a quadword from the $A$ matrix. To use the indexed vector load, we generate indices in lines 5 to 10 and load them into the index vector $index\_vec$. We then utilize the index vector as the second argument when loading data from the $A$ matrix to the $a0\_vec$ vector register. Contrarily, the code snippet demonstrated in algorithm\ref{algo:winogradARMSVE} depicts the execution of tuple multiplication on ARM-SVE. It is evident that in line 7, the "svldrq" vector instruction is employed to fill the vector from the quadword. However, the indexed vector load operation can be cycle-intensive, thereby affecting the overall performance as explained in Section~\ref{results}. We conclude that integrating quadword reading functionality in the "V" extension not only enhances performance but also eliminates the need for workarounds for this operation, simplifying code development.}

  \begin{figure}[!t]
  \centering
  \includegraphics[width=.7\linewidth]{figures/slideup.png}
  \caption{
  Slideup for packing quadword in a 512-bit vector register}
  \label{fig:slideup}
  \vspace{-1.3em}
 \end{figure}
    
    \begin{figure}[!t]
  \centering

    \input{tikz_indexed_load}    
%  \includegraphics[width=.7\linewidth]{figures/tuplemult.png}
  \caption{
  Indexed load for packing quadword in a 512-bit vector register}
  \label{fig:tuplemult}
  \vspace{-1.3em}
 \end{figure}
    
    
    \item[(iii)] For the transformations in the Winograd algorithm, we perform the transpose operation on an array of 4 vectors, as shown in Figure~\ref{fig:tuplemult}.  However  for the  RISC-VV, currently, no specific instructions are available to perform these operations (transposing the two vectors is available as EPI custom extensions~\cite{EPI-builtin}, but not in the standard "V" extension). We, therefore, implement a solution that uses temporary buffers and additional store and gather-load instructions as shown in the algorithm~\ref{algo:transposeriscvv}. To transpose 4 vectors, the process involves storing the vector data into buffer $vin0123$ using memory operations in lines 2 to 5. Subsequently, we generate indices and load them into the $index\_vec$ vector register in lines 8 to 12. Finally, we use an indexed load vector instruction in line 13 to load the transposed values from the buffer into a vector register. 
    
    \deleted{In contrast, when dealing with ARM-SVE, we utilize a combination of "svcreate4" and "svst4" instructions, as demonstrated in lines 2-5 of algorithm\ref{algo:transposeARMSVE}, to generate a tuple of 4 vectors and store the transposed data in the buffer. Further, we use memory load vector instruction to load data from memory to the vector register. Nonetheless, the implementation of the transpose operation of an array of 4 vectors on ARM-SVE also requires memory operation for storing and loading data and these operations can also be cycle-intensive as discussed in section~\ref{results}. }
    
    The requirement of memory operations to store and then gather operations not only put a burden on performance but also decreases programmability, as the developer has to implement more complex solutions. As a result, it would be desirable to extend RISC-VV with an instruction for transposing the four vectors similar to transposing the two vectors and without using any memory operation. 
    
    %As a result, we could have a custom extension in the "V" extension of RISC-V for transposing four vectors in the array of four vectors similar to a custom extension for transposing the two vectors without using any memory operation. 
    
    %of  to create an array of four vectors and then transpose these vectors in the place required in this operation.
    
     \begin{figure}[!t]
  \centering
  \includegraphics[width=.7\linewidth]{figures/tuplevect.png}
  \caption{
  Transpose the elements of vectors}
  \label{fig:tuplevec}
  \vspace{-1.3em}
 \end{figure}

  

  %  \item[(iii)] ISA provides the vector-scalar intrinsics to perform the computations on vector and scalar operands where the operation can be performed on vector register and floating point register. We find this saves the broadcast of the scalar values in vector registers and saves extra instructions. However, to use this feature, it is required for a programmer to use "broadcast" instructions in the program even though these instructions are ignored by the compiler. Therefore, it will be good to have some instructions where programmers can use vector and scalar operand to use the vector-scalar intrinsic instructions. 
\end{enumerate}
    





==> samples <==
% Teach biblatex about numpages field
\DeclareDatamodelFields[type=field, datatype=literal]{numpages}
\DeclareDatamodelEntryfields{numpages}

% Teach biblatex about articleno field
\DeclareDatamodelFields[type=field, datatype=literal]{articleno}
\DeclareDatamodelEntryfields{articleno}

% Teach biblatex about urls field
\DeclareDatamodelFields[type=list, datatype=uri]{urls}
\DeclareDatamodelEntryfields{urls}

% Teach biblatex about school field
\DeclareDatamodelFields[type=list, datatype=literal]{school}
\DeclareDatamodelEntryfields[thesis]{school}

\DeclareDatamodelFields[type=field, datatype=literal]{key}
\DeclareDatamodelEntryfields{key}

% Teach biblatex about lastaccessed field
\DeclareDatamodelFields[type=field,datatype=literal]{lastaccessed}
\DeclareDatamodelEntryfields{lastaccessed}

% Teach biblatex about distincturl field
\DeclareDatamodelFields[type=field, datatype=literal]{distinctURL}
\DeclareDatamodelEntryfields{distinctURL}


%
% include software data model from biblatex-software
%

\blx@inputonce{software.dbx}{biblatex data model extension for software}{}{}{}{}


==> tikz_indexed_load.tex <==
\usetikzlibrary{positioning}
\begin{tikzpicture}[
squarenode/.style={rectangle, draw=blue!60, fill=blue!5, thick, minimum size=5mm},
textnode/.style={rectangle, minimum size=5mm}
]
\node[squarenode] (0) {0};
\node[squarenode] (1) [right=0cm of 0] {1};
\node[squarenode] (2) [right=0cm of 1] {2};
\node[squarenode] (3) [right=0cm of 2] {3};


\node[squarenode] (0_0) [below=of 0] {0};
\node[squarenode] (0_1) [right=0cm of 0_0] {1};
\node[squarenode] (0_2) [right=0cm of 0_1] {2};
\node[squarenode] (0_3) [right=0cm of 0_2] {3};
\node[squarenode] (1_0) [right=0cm of 0_3] {0};
\node[squarenode] (1_1) [right=0cm of 1_0] {1};
\node[squarenode] (1_2) [right=0cm of 1_1] {2};
\node[squarenode] (1_3) [right=0cm of 1_2] {3};
\node[squarenode] (2_0) [right=0cm of 1_3] {0};
\node[squarenode] (2_1) [right=0cm of 2_0] {1};
\node[squarenode] (2_2) [right=0cm of 2_1] {2};
\node[squarenode] (2_3) [right=0cm of 2_2] {3};
\node[squarenode] (3_0) [right=0cm of 2_3] {0};
\node[squarenode] (3_1) [right=0cm of 3_0] {1};
\node[squarenode] (3_2) [right=0cm of 3_1] {2};
\node[squarenode] (3_3) [right=0cm of 3_2] {3};


\node[textnode] () [right=1em of 3] {Index vector};
\node[textnode] () [below=0em of 1_2] {512-bit vector};

\draw[->,blue!60] (0.south) -- (0_0.north);
\draw[->,blue!60] (0.south) -- (1_0.north);
\draw[->,blue!60] (0.south) -- (2_0.north);
\draw[->,blue!60] (0.south) -- (3_0.north);
\end{tikzpicture}

==> tikz_slideup.tex <==
\usetikzlibrary{positioning}
\begin{tikzpicture}[
squarenode/.style={rectangle, draw=blue!60, fill=blue!5, thick, minimum size=5mm},
textnode/.style={rectangle, minimum size=5mm}
]
\node[squarenode] (0) {0};
\node[squarenode] (1) [right=0cm of 0] {1};
\node[squarenode] (2) [right=0cm of 1] {2};
\node[squarenode] (3) [right=0cm of 2] {3};


\node[squarenode] (0_0) [below=of 0] {0};
\node[squarenode] (0_1) [right=0cm of 0_0] {1};
\node[squarenode] (0_2) [right=0cm of 0_1] {2};
\node[squarenode] (0_3) [right=0cm of 0_2] {3};
\node[squarenode] (1_0) [right=0cm of 0_3] {0};
\node[squarenode] (1_1) [right=0cm of 1_0] {1};
\node[squarenode] (1_2) [right=0cm of 1_1] {2};
\node[squarenode] (1_3) [right=0cm of 1_2] {3};
\node[squarenode] (2_0) [right=0cm of 1_3] {0};
\node[squarenode] (2_1) [right=0cm of 2_0] {1};
\node[squarenode] (2_2) [right=0cm of 2_1] {2};
\node[squarenode] (2_3) [right=0cm of 2_2] {3};
\node[squarenode] (3_0) [right=0cm of 2_3] {0};
\node[squarenode] (3_1) [right=0cm of 3_0] {1};
\node[squarenode] (3_2) [right=0cm of 3_1] {2};
\node[squarenode] (3_3) [right=0cm of 3_2] {3};


\node[textnode] () [right=1em of 3] {Index vector};
\node[textnode] () [below=0em of 1_2] {512-bit vector};

\draw[->,blue!60] (0.south) -- (0_0.north);
\draw[->,blue!60] (0.south) -- (1_0.north);
\draw[->,blue!60] (0.south) -- (2_0.north);
\draw[->,blue!60] (0.south) -- (3_0.north);
\end{tikzpicture}

==> tikz_transpose.tex <==
\usetikzlibrary{matrix}
\begin{tikzpicture}[every node/.style={minimum width=1cm, minimum height=1cm, anchor=center}]
  % Array 1
  \matrix (array1) [matrix of nodes, nodes={draw, minimum width=1cm, minimum height=1cm}, column sep=0cm] {
    |[fill=blue!20]| $a_0$ & |[fill=red!20]|$a_1$ & |[fill=green!20]|$a_2$ & |[fill=orange!20]| $a_3$ \\
  };
  \node[left] at (array1.west) {V0};

  % Array 2
  \matrix (array2) [matrix of nodes, nodes={draw, fill=red!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, below of=array1, node distance = 4em] {
    |[fill=blue!20]| $b_0$ & |[fill=red!20]|$b_1$ & |[fill=green!20]|$b_2$ & |[fill=orange!20]| $b_3$ \\
  };
  \node[left] at (array2.west) {V1};

  % Array 3
  \matrix (array3) [matrix of nodes, nodes={draw, fill=green!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, below of=array2, node distance = 4em] {
    |[fill=blue!20]| $c_0$ & |[fill=red!20]|$c_1$ & |[fill=green!20]|$c_2$ & |[fill=orange!20]| $c_3$ \\
  };
  
  \node[left] at (array3.west) {V2};

  % Array 4
  \matrix (array4) [matrix of nodes, nodes={draw, fill=orange!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, below of=array3, node distance = 4em] {
   |[fill=blue!20]| $d_0$ & |[fill=red!20]|$d_1$ & |[fill=green!20]|$d_2$ & |[fill=orange!20]| $d_3$ \\
  };
  \node[left] at (array4.west) {V3};

% Array transpose 1

  \matrix (array1t) [matrix of nodes, nodes={draw, fill=blue!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, right of = array1, node distance = 20em] {
    $a_0$ & $b_0$ & $c_0$ & $d_0$ \\
  };
  \node[left] at (array1t.west) {vin0123[0]};

% Array transpose 2

  \matrix (array2t) [matrix of nodes, nodes={draw, fill=red!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, right of = array2, node distance = 20em] {
    $a_1$ & $b_1$ & $c_1$ & $d_1$ \\
  };
  \node[left] at (array2t.west) {vin0123[1]}; 

  % Array transpose 3

  \matrix (array3t) [matrix of nodes, nodes={draw, fill=green!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, right of = array3, node distance = 20em] {
    $a_2$ & $b_2$ & $c_2$ & $d_2$ \\
  };
  \node[left] at (array3t.west) {vin0123[2]};  

  % Array transpose 2

  \matrix (array4t) [matrix of nodes, nodes={draw, fill=orange!20, minimum width=1cm, minimum height=1cm}, column sep=0cm, right of = array4, node distance = 20em] {
    $a_3$ & $b_3$ & $c_3$ & $d_3$ \\
  };
  \node[left] at (array4t.west) {vin0123[3]};    

\end{tikzpicture}
